Understanding How and Why University Students Use Virtual Private Networks

We study how and why university students chose and use VPNs, and whether they are aware of the security and privacy risks that VPNs pose. To answer these questions, we conducted 32 in-person interviews and a survey with 349 respondents, all university students in the United States. We find students are mostly concerned with access to content and privacy concerns were often secondary. They made tradeoffs to achieve a particular goal, such as using a free commercial VPN that may collect their online activities to access an online service in a geographic area. Many users expected that their VPNs were collecting data about them, although they did not understand how VPNs work. We conclude with a discussion of ways to help users make choices about VPNs.

==> analysis/graphs/q5_14.tex <==
\begin{tabular}{lr}
\toprule
{} & Do you currently use a VPN? \\
\midrule
No  &                         201 \\
Yes &                         148 \\
\bottomrule
\end{tabular}


==> analysis/graphs/q5_16.tex <==
\begin{tabular}{lr}
\toprule
{} & How often do/did you use a VPN when you go online? \\
\midrule
Rarely           &                                                161 \\
Sometimes        &                                                141 \\
Most of the time &                                                 37 \\
Always           &                                                 10 \\
\bottomrule
\end{tabular}


==> analysis/graphs/q7_3.tex <==
\begin{tabular}{lr}
\toprule
{} & Did you read your VPN provider's privacy policy? \\
\midrule
No  &                                              304 \\
Yes &                                               45 \\
\bottomrule
\end{tabular}


==> analysis/graphs/q7_4.tex <==
\begin{tabular}{lr}
\toprule
{} & Do you think your VPN provider collects your data? \\
\midrule
Yes &                                                259 \\
No  &                                                 90 \\
\bottomrule
\end{tabular}

